Synthesis of Sequential Extended Regular Expressions for Verification

Synthesis techniques take realizable Linear Temporal Logic specifications and produce correct cir- cuits that implement the specifications. The generated circuits can be used directly, or as miters that check the correctness of a logic design. Typically, those techniques generate non-deterministic finite state automata, which can be determinized at a possibly exponential cost. Recent results show multiple advantages of using deterministic automata in symbolic and bounded model checking of LTL safety properties. In this paper, we present a technique with a supporting tool that takes a sequential extended regular expression specification {\Phi}, and a logic design implementation S, and generates a sequential circuit C, expressed as an And-Inverted-Graph, that checks whether S satisfies {\Phi}. The technique passes the generated circuit C to ABC, a bounded model checker, to validate correctness. We use free input variables to encode the non- determinism in {\Phi} and we obtain a number of states in miter linear in the size of {\Phi}. Our technique succeeds to generate the input to the model checker while other techniques fail because of the exponential blowup, and in most cases, ABC succeeds to either find defects in the design that was otherwise uncheckable, or validate the design. We evaluated our technique against several industrial benchmarks including the IBM arbiter, a load balancer, and a traffic light system, and compared our results with the NuSMV framework. Our method found defects and validated systems NuSMV could not validate.

==> proof.tex <==
%%% proof of equisatisfiability
In this appendix, we present an inductive proof of Theorem~\ref{thm:equisat}
presented in section~\ref{s:core}.
We will prove Theorem~\ref{thm:equisat} by first proving the more constrained Lemma~\ref{lemma:constr_equisat},
which states that the formula $\psi$ and the constructed DFA $M$ are equisatisfiable, and that for each 
trace $\rho$ that satisifies $\psi$, there exists a trace $\rho'$ of equal length that satisfies $M$, and vice versa, 
where the length of a trace $\rho$ is the number of valuations in the sequence, denoted by $|\rho|$. 

%% Theorem 1 
%\begin{theorem} \label{th:equisat}
% Let $\psi$ be an SERE formula and $M = (Q, I, F, \delta, \eval)$ such that $Q$, $I$, $F$, and $\delta$
%are constructed according to equation~\ref{eq:construct}. Then $\psi$ and $M$ are equisatisfiable, 
%i.e. $\exists{\rho},~\rho \models \psi \Leftrightarrow \exists{\rho'},~\rho' \models M$.  
%\end{theorem}

\begin{lemma}[Constrained equisatisfiability of $M$ and $\psi$]
\label{lemma:constr_equisat}
Let $\psi = x_1y_1;x_2y_2;\ldots;x_ny_n$ be a SERE formula, and $M = (Q, I, F, \mathbb{V}', \mathbb{T}', \delta)$
be the corresponding constructed DFA, then $\psi$ and $M$ are equisatisfiable and for each trace that
satisifes $\psi$ corresponds a trace of equal length that satisifes $M$, and vice versa. That is
$\exists{\rho},~\rho \models \psi \Leftrightarrow \exists{\rho'},~\rho' \models M \land |\rho| = |\rho'|$.  
\end{lemma}

%% Start of proof
The base case in our proof consists of the case where the length of the SERE formula $\psi$ is 1, that is 
$\psi = x_1y_1$, $x_1 \in \mathbb{T}$ and $y_1 \in \{\epsilon, *\}$. To prove the constrained equisatisfiability of 
$\psi$ and the constructed DFA $M$, we consider two cases each corresponding to $y_1$ being $\epsilon$ and $*$ 
respectively.

\noindent{ {\bf Case 1}} $y_1 = \epsilon$. 

{\bf a.} $\exists{\rho},~\rho \models \psi \rightarrow \exists{\rho'},~\rho' \models M \land |\rho| = |\rho'|$. 
\begin{proof}
We know that $\rho \models \psi \rightarrow \rho = v_1 \land (v(x_1)=\cci{true}), v_1 \in \mathbb{V}$.
By construction of $M$, we have that 
$Q = \{s_0, s_1\}$, %
$I = \{s_0\}$, %
$F = \{s_1\}$, and %
$\delta = \{(s_0, r \land x_1, s_1), (s_0, \lnot r, s_0)\}$. 
%\begin{equation}
%\left\{
%        \begin{array}{l}
%                Q = \{s_0, s_1\} \\
%                I = \{s_0\} \\
%                F = \{s_1\} \\
%                \delta = \{(s_0, s_1, r \land x_1), (s_0, s_0, \lnot r), (s_1, s_0, 1)\} 
%        \end{array} \right .
%\end{equation}
Let $\rho' = u_1$ with $u_1 \in \eval'$ such that $u_1 = v_1 \cup \{(r, \mbox{\cci{true}})\}$.
$\rho' \models M$ since it will exercise the transition $(s_0, x_1 \land r, s_1)$, 
and $s_1 \in F$. Additionally, we have that $|\rho| = |\rho'| = 1$. 
\end{proof}

{\bf b.} $\exists{\rho'},~\rho' \models M \rightarrow \exists{\rho},~\rho \models \psi \land |\rho| = |\rho'|$.
\begin{proof}
$\rho' \models M \rightarrow \exists{i}\in [1 \ldots |\rho'|].\rho'(x_1 \land r, i) = \mbox{\cci{true}}$. 
Let $\rho' = \rho'_i$ then $|\rho'| = 1$. Also let $\rho = \rho' - \{(r, \mbox{\cci{true}}), (r, \mbox{\cci{false}})\}$, then 
$|\rho| = 1 \land \rho(x_1, 1) = \mbox{\cci{true}}$, therefore $\rho \models \psi \land |\rho| = |\rho'| = 1$.
\end{proof}

{\bf c.} $\nexists{\rho},~\rho \models \psi \rightarrow \nexists{\rho'},~\rho' \models M$.
\begin{proof}
Given that $\nexists{\rho}.\rho \models \psi$, assume that $\exists{\rho'}.\rho' \models M$. 
Then by part (b), $\exists{\rho}.\rho \models \psi$ which is a contradiction. Therefore we can conclude that 
$\nexists{\rho'},~\rho' \models M$.
\end{proof}

{\bf d.} $\nexists{\rho'},~\rho' \models M \rightarrow \nexists{\rho},~\rho \models \psi$.
\begin{proof}
Given that $\nexists{\rho'}.\rho' \models M$, assume that $\exists{\rho}.\rho \models \psi$. 
Then by part (a), 
$\exists{\rho'}.\rho' \models M$ which is a contradiction. Therefore we can conclude that 
$\nexists{\rho}.\rho \models \psi$.
\end{proof}

\noindent {{\bf Case 2:}} $y_1 = *$.
\begin{proof}
The proof in this case relies on the fact that $\psi = x_1* \rightarrow \forall \mbox{trace } \rho. \rho \models \psi$,
since any trace $\rho$ satisifies $x_1$ at least 0 times. We say in this case that $\psi$ is universe.
%Let $\sigma \in \eval$ be the valuation $\set{(x_1,\mbox{\cci{true}})}$, and $\rho^0 = \epsilon$.
%We define $\rho^1 = \rho^0\circ\sigma$, 
%$\rho^2 = \rho^1\circ\sigma = \rho^0\circ\sigma\circ\sigma$, and $\rho^{n+1} = \rho^{n-1}\circ\sigma, n \in \mathbb{N}$. 
%$\rho \models x_1* \Leftrightarrow 
%(\rho = \rho^0) \lor (\rho = \rho^1) \lor \ldots \lor (\rho = \rho^i) \lor \ldots, i \in \mathbb{N}$.
%
%Assume $\rho \nvdash x_1*$ for some trace $\rho$. Therefore from the above definition
%$\rho = \lnot(\rho^0 \lor \rho^1 \lor \rho^2 \lor \ldots) = (\lnot \rho^0 \land \lnot \rho^1 \land \lnot \rho^2 \ldots)$. 
%But $\rho = (\lnot \rho^1 \land \lnot \rho^2 \land \ldots) \rightarrow \rho \nvdash x_1 \lor \rho = \epsilon$, which 
%is the definition of $\rho_0$. Therefore $\rho = \lnot \rho^0 \land \rho^0$ which is never satisfiable, therefore 
%$\nexists{\rho},~\rho \nvdash x_1* \Leftrightarrow \psi \mbox{ is universe}$. \newline
By construction of $M$, we have that $Q = \{s_0, s_1\}, %
                I = \{s_0\}, %
                F = \{s_0, s_1\}$, and %  \\
                $\delta =  \{ (s_0, \lnot r, s_0), (s_0, x_1 \land r, s_1), (s_1, x_1, s_1), (s_1, \lnot x_1, s_0) \}$.
Since $F = Q$ then $M$ accepts any input trace, that is $M$ is also universe. 
Therefore for any trace $\rho$ such that $\rho \models \psi$, we let $\rho' = \rho$, then $\rho' \models M \land |\rho'| = |\rho|$. 
\end{proof}

\noindent {\bf Inductive hypothesis.} 
Let $n \in \mathbb{N}, n \geq 1$, $\psi = x_1y_1;\ldots;x_ny_n$, and $M_\psi$ be the corresponding constructed DFA. 
Also let $\phi = \psi;x_{n+1}y_{n+1}$ and $M_\phi$ be the corresponding constructed DFA. 
Assume that $\psi$ and $M_\psi$ are equisatisfiable and have the constraint of Lemma~\ref{lemma:constr_equisat}.
We now have to prove that $\phi$ and $M_\phi$ are also equisatisfiable under the constraint of Lemma~\ref{lemma:constr_equisat}.
We consider three different cases depending on the values of $y_n$ and $y_{n+1}$.

\noindent {{\bf Case 1:}} $y_n = \epsilon \land y_{n+1} = \epsilon$. \\
By construction of $M_\phi$, we have that $Q_\phi = Q_\psi \cup \set{s_{n+1}}$, 
$I_\phi = I_\psi$, and $F_\phi = \set{s_{n+1}}$. The transition function $\delta_\phi$
of $M_\phi$ is related to $\delta_\psi$ as follows:
$$\delta_\phi = \delta_\psi \cup \set{(s_n, x_{n+1}, s_{n+1}), (s_n, \lnot x_{n+1}, s_0)}$$

{\bf a.} $\exists{\rho},~\rho \models \phi \rightarrow \exists{\rho'},~\rho' \models M_\phi \land |\rho| = |\rho'|$.
\begin{proof}
Let $\rho_1 \models \psi$, then by the inductive hypothesis we have that $\exists{\rho'_1}.\rho'_1 \models M_\psi$
with $|\rho_1| = |\rho'_1|$.
Let $\rho = \rho_1\circ\rho_2$ such that $\rho \models \phi$, therefore $\rho_2 \models x_{n+1}$.
We construct $\rho'$ such that $\rho' = \rho'_1\circ\rho'_2$ with $\rho'_2 = \rho_2$, therefore $\rho'$ exercises the 
transition $(s_n, x_{n+1}, s_{n+1})$ which implies that $\rho' \models M_\phi \land |\rho'| = |\rho| = |\rho_1| + |\rho_2|$.
\end{proof}

{\bf b.} $\exists{\rho'},~\rho' \models M_\phi \rightarrow \exists{\rho},~\rho \models \phi \land |\rho'| = |\rho|$.
\begin{proof}
Let $\rho'_1 \models M_\psi$, then by the inductive hypothesis we have that $\exists{\rho_1}.\rho_1 \models M_\phi$
with $|\rho_1| = |\rho'_1|$.
Let $\rho' = \rho'_1\circ\rho'_2$ such that $\rho' \models M_\phi$, therefore 
$\rho'_2 \models x_{n+1}$.
We construct $\rho$ such that $\rho = \rho_1\circ\rho_2$ with $\rho_2 = \rho'_2$, therefore 
$\rho_2 \models x_{n+1}$ and $\rho \models \phi$ since $\rho_1 \models \psi$,
with $|\rho| = |\rho'| = |\rho_1| + |\rho_2|$.
\end{proof}

{\bf c.} $\nexists{\rho},~\rho \models \phi \rightarrow \nexists{\rho'},~\rho' \models M_\phi$. 
\begin{proof}
Given $\nexists{\rho},~\rho \models \phi$, assume that $\exists{\rho'}.~\rho' \models M_\phi$, then by part (b)
we have that $\exists{\rho},~\rho \models \phi$ which is a contradiction.
Therefore $\nexists{\rho'},~\rho' \models M_\phi$.
\end{proof}

{\bf d.} $\nexists{\rho'},~\rho' \models M_\phi \rightarrow \nexists{\rho},~\rho \models \phi$. 
\begin{proof}
Given $\nexists{\rho'}.\rho' \models M_\phi$, assume that $\exists{\rho}.\rho \models \phi$, then by part (a)
we have that $\exists{\rho'}.\rho' \models M_\phi$ which is a contradiction.
Therefore $\nexists{\rho}.\rho \models \phi$. 
\end{proof}

\noindent {{\bf Case 2:}} $y_{n+1} = *$. \\
Let $m$ be the number of consecutive $*$ operators ending with $y_{n+1}$, and 
$S^* = \set{s_{n-m+2}, s_{n-m+3}, \ldots, s_{n+1}}$ be the $m$ corresponding states. 
$choice(k,p,\bar{r})$ is defined as in section~\ref{s:core}.

By construction of $M_\phi$, we have that $Q_\phi = Q_\psi \cup \set{s_{n+1}}$, 
$I_\phi = I_\psi$, and $F_\phi = F_\psi \cup \set{s_{n+1}}$. The transition relation 
$\delta_\phi$ of $M_\phi$ is related to the transition relation $\delta_\psi$ of $M_\psi$
as follows:
\parbox{2.8in}{ \begin{tabbing}
mm\=mm\=mm\=mm\=mm \kill
$\delta_\phi$ \>$=$ \> $\delta_\psi - \{(s_i, \_\_, \_\_)~|~ s_i \in S^* \lor s_i = s_{n-m+1}\}$ \\
\> $\cup$ \> $\{ (s_i, \bigwedge_{j=i}^{n+1} \lnot x_j, s_0)~|~ s_i \in S^* \lor s_i = s_{n-m+1}\}$ \\
\> $\cup$ \> $\{ (s_i, x_j \land ( choice(i,j,\bar{r}) \lor (\lnot x_i \land \bigwedge_{k=j+1}^{n+1} \lnot x_k) ), s_j )$ \\
\> \> \> $|~ s_i \in S^* \lor s_i = s_{n-m+1} \land i < j \leq n+1 \}$ \\
\> $\cup$ \> $\{ (s_i, x_i \land ( choice(i,i,\bar{r}) \lor \bigwedge_{k=i+1}^{n+1} \lnot x_k ), s_i )| s_i \in S^* \}$ \\
\end{tabbing}
}

{\bf a.} $\exists{\rho},~\rho \models \phi \rightarrow \exists{\rho'},~\rho' \models M_\phi \land |\rho| = |\rho'|$.
\begin{proof}
Let $\rho_1 \models \psi$ then by the inductive hypothesis we have that $\exists{\rho_1'},~\rho_1' \models M_\psi$. 
Let $\rho = \rho_1\circ\rho_2$ such that $\rho \models \phi$, then we have that $\rho_2 \models x_{n+1}*$. 
We will differentiate between two cases:
\begin{enumerate}
 \item $|\rho_2| = 0$. 
 Let $\rho' = \rho'_1$, then $\rho' \models M_\phi$ and $|\rho'| = |\rho|$. Note that although in this case, the 
 state $s_{n+1}$ is not reached, the DFA $M_\phi$ still accepts the input since $F_\phi = F_\psi \cup \set{s_{n+1}}$, so
 $\rho'_1$ will cause a set of transitions that will lead $M_\phi$ into a state $s \in F_\psi$ since $\rho'_1 \models M_\psi$.
 
 \item $|\rho_2| \geq 1$. 
 In this case, we have that $\rho_2 \models x_{n+1}$ at least once. Let $\rho' = \rho'_1\circ\rho'_2$ such that 
 $\rho'_2 = \rho_2$ with $choice(k,n+1,\bar{r})$ added as a conjuction to each valuation in $\rho_2$,
 where $k$ is the index of the last state that $\rho'_1$ reaches.
 Since $\rho'_1 \models M_\psi$, $s_k$ is guaranteed to be one of the accept states of $M_\psi$ as all the transitions
 of $M_\psi$ are preserved in $M_\phi$. Although this is enough to say that $\rho' \models M_\phi$, we emphasize that
 $M_\phi$ will also transition into the state $s_{n+1}$, providing an accurate translation of $\phi$. 
 Therefore $\rho' \models M_\phi \land |\rho'| = |\rho| = |\rho'_1| + |\rho'_2|$.
\end{enumerate}
\end{proof}

{\bf b.} $\exists{\rho'},~\rho' \models M_\phi \rightarrow \exists{\rho},~\rho \models \phi \land |\rho'| = |\rho|$.
\begin{proof}
Let $\rho'_1 \models M_\psi$ then by the inductive hypothesis we have that 
$\exists{\rho_1}.\rho_1 \models \psi \land |\rho_1| = |\rho'_1|$.
Let $\rho' = \rho'_1\circ\rho'_2$ such that $\rho' \models M_\phi$.
We will differentiate between two different cases:
\begin{enumerate}
 \item $|\rho'_2| = 0$. We construct $\rho = \rho_1$ and it's a direct implication that $\rho \models \phi$ since 
 $\rho_1 \models \psi$, and $|\rho| = |\rho'|$.
 \item $|\rho'_2| \geq 1$. Let $\rho = \rho_1\circ\rho_2$ such that $\rho_2 = \rho'_2$ with all additional atomic 
 propositions $\bar{r}$ removed from the valuations of $\rho'_2$. Although the additional atomic propostitions are removed, 
 $\rho_2$ still satisfies $x_{n+1}$ at least once, then $\rho_2 \models x_{n+1}*$. Therefore $\rho \models \phi$ since
 $\rho_1 \models \psi$ and $\rho_2 \models x_{n+1}*$. Additionally, $|\rho| = |\rho'| = |\rho'_1| + |\rho'_2|$.
\end{enumerate} 
\end{proof}

{\bf c.} $\nexists{\rho},~\rho \models \phi \rightarrow \nexists{\rho'},~\rho' \models M_\phi$. 
\begin{proof}
Given $\nexists{\rho}.\rho \models \phi$, assume that $\exists{\rho'}.\rho' \models M_\phi$, then by part (b)
we have that $\exists{\rho}.\rho \models \phi$ which is a contradiction.
Therefore $\nexists{\rho'}.\rho' \models M_\phi$.
\end{proof}

{\bf d.} $\nexists{\rho'},~\rho' \models M_\phi \rightarrow \nexists{\rho},~\rho \models \phi$. 
\begin{proof}
Given $\nexists{\rho'}.\rho' \models M_\phi$, assume that $\exists{\rho}.\rho \models \phi$, then by part (a)
we have that $\exists{\rho'}.\rho' \models M_\phi$ which is a contradiction. \\
Therefore $\nexists{\rho}.\rho \models \phi$.
\end{proof}

\noindent {{\bf Case 3:}} $y_n = * \land y_{n+1} = \epsilon$. \\
Let $m$ be the number of consecutive $*$ operators ending with $y_{n}$, and 
$S^* = \set{s_{n-m+1}, s_{n-m+2}, \ldots, s_{n}}$ be the $m$ corresponding states. 
$choice(k,p,\bar{r})$ is defined as in section~\ref{s:core}.

By construction of $M_\phi$, we have that $Q_\phi = Q_\psi \cup \set{s_{n+1}}$, 
$I_\phi = I_\psi$, and $F_\phi =\set{s_{n+1}}$. The transition relation 
$\delta_\phi$ of $M_\phi$ is related to the transition relation $\delta_\psi$ of $M_\psi$
as follows:
\parbox{2.8in}{ \begin{tabbing}
mm\=mm\=mm\=mm\=mm \kill
$\delta_\phi$ \>$=$ \> $\delta_\psi - \{(s_i, \_\_, \_\_)~|~ s_i \in S^* \lor s_i = s_{n-m}\}$ \\
\> $\cup$ \> $\{ (s_i, \bigwedge_{j=i}^{n+1} \lnot x_j, s_0)~|~ s_i \in S^* \lor s_i = s_{n-m}\}$ \\
\> $\cup$ \> $\{ (s_i, x_j \land ( choice(i,j,\bar{r}) \lor (\lnot x_i \land \bigwedge_{k=j+1}^{n+1} \lnot x_k) ), s_j )$ \\
\> \> \> $|~ s_i \in S^* \lor s_i = s_{n-m} \land i < j \leq n \}$ \\
\> $\cup$ \> $\{ (s_i, x_i \land ( choice(i,i,\bar{r}) \lor \bigwedge_{k=i+1}^{n+1} \lnot x_k ), s_i )| s_i \in S^* \}$ \\
\end{tabbing}
}

{\bf a.} $\exists{\rho},~\rho \models \phi \rightarrow \exists{\rho'},~\rho' \models M_\phi \land |\rho| = |\rho'|$.
\begin{proof}
Let $\rho_1 \models \psi$ then by the inductive hypothesis $\exists{\rho'_1}.\rho'_1 \models M_\psi$. 
Let $\rho = \rho_1\circ\rho_2$ such that $\rho \models \phi$ then by the semantics of SERE we have
$\rho_2 \models x_{n+1}$.
Since $|\rho_2| = 1 \geq 1$, we can reason in the same way as in case 2, part (a) and prove
that $\exists{\rho'}.\rho' \models M_\phi \land |\rho'| = |\rho|$.
\end{proof}

{\bf b.} $\exists{\rho'},~\rho' \models M_\phi \rightarrow \exists{\rho},~\rho \models \phi \land |\rho'| = |\rho|$.
\begin{proof}
Let $\rho'_1 \models M_\psi$ then by the inductive hypothesis $\exists{\rho_1}.\rho_1 \models \psi$. 
Let $\rho'_1 = \rho'_1\circ\rho'_2$ such that $\rho' \models M_\phi$, then by the construction of $M_\phi$, $\rho'_2$ is of the form
$|\rho'_2| = 1 \land |\rho'_2| \models x_{n+1}$. 
Let $\rho = \rho_1\circ\rho_2$ such that $\rho_2 = \rho'_2$ with the additional atomic propositions $\bar{r}$ removed, 
we will still have that $\rho_2 \models x_{n+1}$. Since $\rho_1 \models \psi \land \rho_2 \models x_{n+1}$,
$\rho \models \phi$, and $|\rho| = |\rho'| = |\rho'_1| + |\rho'_2|$.
\end{proof}

{\bf c.} $\nexists{\rho},~\rho \models \phi \rightarrow \nexists{\rho'},~\rho' \models M_\phi$. 
\begin{proof}
Given $\nexists{\rho}.\rho \models \phi$, assume that $\exists{\rho'}.\rho' \models M_\phi$, then by part (b)
we have that $\exists{\rho}.\rho \models \phi$ which is a contradiction.
Therefore $\nexists{\rho'}.\rho' \models M_\phi$. \newline
\end{proof}

{\bf d.} $\nexists{\rho'},~\rho' \models M_\phi \rightarrow \nexists{\rho},~\rho \models \phi$. 
\begin{proof}
Given $\nexists{\rho'}.\rho' \models M_\phi$, assume that $\exists{\rho}.\rho \models \phi$, then by part (a)
we have that $\exists{\rho'}.\rho' \models M_\phi$ which is a contradiction. 
Therefore $\nexists{\rho}.\rho \models \phi$. \newline 
\end{proof}

This concludes the proof of Lemma~\ref{lemma:constr_equisat}. It is easy to see that Lemma~\ref{lemma:constr_equisat}
directly implies Theorem~\ref{thm:equisat}, which concludes our proof of correctness for the equisatisfiable DFA construction. 


%\begin{equation} \label{eq:star}
% \rho \models \psi \rightarrow \left\{
%	 \begin{array}{l l}
%		\rho = \epsilon & (a)\\
%		\rho = 1 \land \rho = v_1 \land v_1(x_1) & (b) \\
%		\rho = 1 \land \rho = v_1 \land \lnot v_1(x_1) & (c) \\
%		|\rho| = 1 \land \rho = \rho_1\rho_2 \land \rho_1 = v_1 \land
%		v_1(x_1) \land \rho_2 \models \psi & (d)
%	 \end{array} \right .
%\end{equation}

%Let $\psi = x_1y_1$ with $y_1 = \epsilon$, and let $M$ be the DFA constructed according to 
%the algorithm presented in section~\ref{s:construction}. We need to prove that $\psi$ and $M$
%are equisatisfiable, i.e. $\exists{\rho},~\rho \models \psi \Leftrightarrow \exists{\rho'},~\rho' \models M$. 
%
%%% Step 1
%\begin{lemma} \label{l:1.1}
%$\exists{\rho},~\rho \models \psi \rightarrow \exists{\rho'},~\rho' \models M$.
%\end{lemma}
%
%\begin{proof}
%$\rho \models \psi \rightarrow |\rho| = 1 \land \rho = v_1 \land v_1(x_1)$.\\
%Let $\rho' = u_1$ with $u_1 = v_1 \union \{(r, \mbox{\texttt{true}})\}$. 
%By construction of $M$, we have that $\rho' \models M$.  
%\end{proof}
%
%%% Step 2 
%\begin{lemma} \label{l:1.2}
%$\exists{\rho'},~\rho' \models M \rightarrow \exists{\rho},~\rho \models \psi$.
%\end{lemma}
%
%\begin{proof}
%$\rho' \models M \rightarrow \exists{i},~ i \in [0 \ldots |\rho'|] ~s.t.~ \rho'_i = u_i \land u_i(x_1) \land u_i(r)$.\\
%Let $v_1 = u_1 - \{(r, \mbox{\texttt{true}}), (r, \mbox{\texttt{false}})\}$ with $v_1(x_1) = \mbox{\texttt{true}}$.
%Let $\rho = v_1$ then $\rho \models \psi$.   
%\end{proof}
%
%%% Step 3
%\begin{lemma} \label{l:1.3}
%$\nexists{\rho},~\rho \models \psi \rightarrow \nexists{\rho'},~\rho' \models M$.
%\end{lemma}
%
%\begin{proof}
%Assume that $\rho' \models M$. By lemma~\ref{l:1.2}, $\exists{\rho},~\rho \models \psi$, which is
%a contradiction to the first part of the implication. Therefore $\nexists{\rho'},~\rho' \models M$. 
%\end{proof}
%
%%% Step 4 
%\begin{lemma} \label{l:1.4}
%$\nexists{\rho'},~\rho' \models M \rightarrow \nexists{\rho},~\rho \models \psi$.
%\end{lemma}
%
%\begin{proof}
% Assume that $\rho \models \psi$. By lemma~\ref{l:1.1}, $\exists{\rho'},~\rho' \models M$, which is
%a contradiction. Therefore $\nexists{\rho},~\rho \models \psi$.
%\end{proof}
%
%%% Theorem 1
%\begin{theorem} \label{th:base}
%$\psi = x_1y_1,~y_1 = \epsilon \rightarrow ( \exists{\rho},~\rho \models \psi \Leftrightarrow \exists{\rho'},~\rho' \models M )$
%\end{theorem}
%
%\begin{proof}
%The proof follows directly from lemmas~\ref{l:1.1} to~\ref{l:1.4}.
%\end{proof}
%
%
%Now let $\psi = x_1y_1$ with $y_1 = *$, and let $M$ be the DFA constructed
%from $\psi$ according to the algorithm previousely presented. 
%
%%% step 0 : universe
%\begin{lemma} \label{l:2.0}
% $\psi = x_1* \rightarrow \psi \mbox{ is universe.}$
%\end{lemma}
%
%\begin{proof}
%\begin{equation} \label{eq:star}
% \rho \models \psi \rightarrow \left\{
%	 \begin{array}{l l}
%		\rho = \epsilon & (a)\\
%		\rho = 1 \land \rho = v_1 \land v_1(x_1) & (b) \\
%		\rho = 1 \land \rho = v_1 \land \lnot v_1(x_1) & (c) \\
%		|\rho| = 1 \land \rho = \rho_1\rho_2 \land \rho_1 = v_1 \land
%		v_1(x_1) \land \rho_2 \models \psi & (d)
%	 \end{array} \right .
%\end{equation}
%
%Assume $\exists{\rho}~,\rho \nvdash \psi$, then it is certain that $\rho \neq \epsilon$. 
%According to the definition in equation~\ref{eq:star}, $\rho \nvdash \psi \rightarrow$ $\rho$ is
%not of the form (a), nor (b), nor (c), i.e. $\rho \neq (a) \land \rho \neq (b) \land \rho \neq (c)$. 
%Assume $\rho \models \psi \land \rho \neq (a)$, therefore $|\rho| = 1 \land \rho = v_1 \land \lnot v_1(x_1)$, but then $\rho$
%is of the form $(c)$, so $\rho \models \psi$ which is a contradiction. Therefore the equation 
%$\rho \neq (a) \land \rho \neq (b) \land \rho \neq (c)$ is never satisfiable and thus $\psi$ is universe.  
%\end{proof}
%
%\begin{theorem}
% Let $\psi = x_1*$ and $M = DFA(\psi)$, then $\exists{\rho},~\rho \models \psi \Leftrightarrow \exists{\rho'},~\rho' \models M$.
%\end{theorem}
%
%\begin{proof}
% By lemma~\ref{l:2.0}, $\psi$ is universe. And by construction, $M$ is universe since it is always accepting. Any $\rho$ that 
%models $\psi$ is directly acceptable by $M$ and vice versa. Therefore $\psi$ and $M$ are equisatisfiable. Note that since $\psi$ 
%is universe, $\nexists{\rho},~\rho \nvdash \psi$. 
%\end{proof}
%%%%%%%%%%%%%
%
%Let $\phi = \psi;x_{n+1}y_{n+1}$ where $\psi$ is a SERE formula of the form $x_1y_1, x_2y_2, \ldots, x_n,y_n$, and let $M$ be 
%the DFA generated by applying algorithm presented in section~\ref{s:construction}. Also, let $\mphi$ and $\mpsi$ be the DFAs 
%constructed from $\phi$ and $\psi$ respectively. We will use induction to prove that $\phi$ and $\mphi$ are equisatifiable. 
%
%The base case is when $\psi = \epsilon$, this has been proven using theorem~\ref{th:base}. Now for some scalar value $n \geq 0$, 
%let $\psi = x_1y_1;\ldots;x_ny_n$ and assume that $\psi$ and $\mpsi$ are equisatisfiable.
%We need to prove that $\phi = \psi;x_{n+1}y_{n+1}$ and $\mphi$ are equisatisfiable. We will consider four cases depending on what 
%$y_n$ and $y_{n+1}$ are. 
%
%\begin{lemma} \label{l:3.0}
%$\exists{\rho},~\rho \models \phi \Leftrightarrow \exists{\rho'},~\rho' \models \mphi$ 
%\end{lemma}
%
%%\begin{proof}
%\paragraph{Case 1:}$y_n = \epsilon$ and $y_{n+1} = \epsilon$.
%Let $\mpsi = (Q_1, I_1, F_1, \delta_\psi, L_1)$. By construction we have $\mphi = (Q, I, F, \delta, L)$ such that:
% 
%\begin{itemize}
% \item $Q = Q_1 \union~\{ s_{n+1} \}$
% \item $I = I_1$
% \item $F = \{ s_{n+1} \}$
% \item $\delta = ( \delta_\psi - \{ (s_n, s_0, 1) \} )~\union~\{ (s_n, s_{n+1}, x_{n+1}), (s_{n+1}, s_1, 1) \}$ 
%\end{itemize}
%
%Let $\rho_1 \models \psi$, $\rho = \rho_1\rho_2 \models \mphi$ and $\rho'_1 \models \mpsi$. We define $\rho' = \rho'_1\rho'_2$ such that 
%$\rho'_2 = \rho_2$, then by construction of $\mphi$, $\rho' \models \mphi$ since $\rho'_1$ will move $\mphi$ to $s_n$ and then $\rho'_2$
%will move the DFA to $s_{n+1} \in F$. 
%%\end{proof}
%
%\paragraph{Case 2:}$y_n = \epsilon$ and $y_{n+1} = \epsilon$.
%Let $\mpsi = (Q_1, I_1, F_1, \delta_\psi, L_1)$. By construction we have $\mphi = (Q, I, F, \delta, L)$ such that:
%\begin{itemize}
% \item $Q = Q_1 \union~\{ s_{n+1} \}$
% \item $I' = I$
% \item $F' = F \union \{ s_{n+1} \}$
% \item $\delta = ( \delta_\psi - \{ (s_n, s_0, 1) \} )~\union~\{ (s_n, s_{n+1}, x_{n+1}), (s_{n+1}, s_{n+1}, x_{n+1}), ( s_{n+1}, s_0, \lnot x_{n+1}), 
% ( s_n, s_0, \lnot x_{n+1} ) \}$
%\end{itemize}
%
%Let $\rho_1 \models \psi$, since $x_{n+1}*$ is universe, $\forall{\rho_2},~\rho = \rho_1\rho_2 \models \psi$. Then, given $\rho_1' \models \mpsi$, 
%$\forall{\rho'_2}~\rho' = \rho'_1\rho'_2 \models \mphi$. In other words, any trace $\rho'_1$ that satisfies $\mpsi$ will also satisfy $\mphi$. Additionally, 
%any trace $\rho' = \rho'_1\rho'_2$ will also satisfy $\mphi$ for all trace $\rho'_2$.
%
%\paragraph{Case 3:}$y_n = *, y_{n+1} = *$. 
%Similarly to case (2), $x_{n+1}y_{n+1}$ is universe and we can apply the same proof previously used to prove that 
%$\exists{\rho}~\rho \models \phi \rightarrow \exists{\rho'}~\rho' \models \mphi$.
%
%\paragraph{Case 4:}$y_n = *, y_{n+1} = \epsilon$.
%Let $\mpsi = (Q_1, I_1, F_1, \delta_\psi, L_1)$. By construction we have $\mphi = (Q, I, F, \delta, L)$ such that:
%\begin{itemize}
% \item $Q = Q_1 \union~\{ s_{n+1} \}$
% \item $I' = I$
% \item $F' = \{ s_{n+1} \}$
% \item $\delta = ( \delta_\psi - \{ (s_n, s_0, \lnot x_n), (s_{n-1}, s_n, x_n), (s_n, s_n, x_n) \} )~\union~\{ (s_n, s_{n+1}, 
% (x_{n+1} \land r) \lor (x_{n+1} \land \lnot x_n)),
% (s_n, s_n, (x_n \land \lnot r) \lor ( x_n \land \lnot x_{n+1} )), (s_{n+1}, s_0, 1), ( s_n, s_0, \lnot x_n \land x_{n+1} ), 
% (s_{n-1}, s_{n+1}, (x_{n+1} \land r) \lor ( x_{n+1} \land \lnot x_n) ), 
% (s_{n-1}, s_n, (x_n \land \lnot r) \lor (x_n \land \lor x_{n+1}),
% (s_{n-1}, s_0, \lnot x_n \land \lnot x_{n+1}) \}$ 
%\end{itemize}
%
%Given $\rho_1 \models \mphi$, $\rho = \rho_1\rho_2 \models \mpsi$ and $\rho'_1 \models \mpsi$. 
%Let $\rho'_2 = \rho_2 \union \{ (r, \mbox{\texttt{true}})\}$, therefore $\rho' = \rho'_1\rho'_2 \models \mphi$.  
%Note that $\mphi$ can reach the accept state $s_{n+1}$ by two ways, either from $s_n$ or from $s_{n+1}$ and both these
%ways are captured by the proposition $(x_{n+1} \land r) \lor (x_{n+1} \land \lnot x_n)$.
%
%\begin{lemma} \label{l:3.1}
%$\exists{\rho'}~\rho' \models \mphi \rightarrow \exists{\rho}~\rho \models \phi$. 
%\end{lemma}
%
%\paragraph{Case 1:}$y_n = \epsilon, y_{n+1} = \epsilon$.
%The construction for $\mphi$ from $\mpsi$ is the same as the one used in the previous proof. 
%We have established from before that $\exists{\rho'_1}~\rho'_1 \models \mpsi \rightarrow \exists{\rho',\rho'_2}~\rho'=\rho'_1\rho'_2 \models \mphi$ such 
%that $|\rho'_2| = 1 \land \rho'_2 = v \land v(x_1)$. 
%
%Also by our inductive assumption, $\rho'_1 \models \mpsi \rightarrow \exists{\rho_1}~\rho_1 \models \psi$. 
%Let $\rho_2 = \rho'_2$, then $\rho = \rho_1\rho_2 \models \phi$. 
%
%\paragraph{Case 2:}$y_n = \epsilon, y_{n+1} = *$.
%Let $\rho' \models \mphi$, therefore by construction $\exists{\rho'_1}~\rho'_1 \models \mpsi$ and by our inductive 
%assumption $\exists{\rho_1}~\rho_1 \models \psi$. 
%Since $y_{n+1} = *$, $x_{n+1}y_{n+1}$ is universe and thus $\forall{\rho_2}~\rho = \rho_1\rho_2 \models \phi$. 
%
%\paragraph{Case 3:}$y_n = *, y_{n+1} = *$. 
%The proof for this case follows directly from the proof for case 2. 
%
%\paragraph{Case 4:}$y_n = *, y_{n+1} = \epsilon$. 
%Let $\rho'_1 \models \mpsi$, then by construction $\rho' = \rho'_1\rho'_2 \models \mphi$ where 
%$\rho'_2 = v \land v((x_{n+1} \land r) \lor (x_{n+1} \land \lnot x_n))$. Also by our inductive assumption, 
%$\exists{\rho_1}~\rho_1 \models \psi$. 
%
%Let $\rho_2 = \rho'_2 - {(r, \mbox\{\texttt{true}}), (r, \mbox{\texttt{false}})\}$ then $\rho = \rho_1\rho_2 \models \phi$. 
%
%
%\begin{lemma} \label{l:3.2}
% $\nexists{\rho}~\rho \models \phi \rightarrow \nexists{\rho'}~\rho' \models \mphi$.
%\end{lemma}
%
%\begin{proof}
%Assume $\rho' \models \mphi$, then by lemma~\ref{l:3.1}, $\exists{\rho}~\rho \models \phi$ which is a 
%contradiction to the left hand side of the implication ($\nexists{\rho}~\rho \models \phi$), and thus 
%such a $\rho'$ does not exist. 
%\end{proof}
%
%\begin{lemma} \label{l:3.3}
% $\nexists{\rho'}~\rho' \models \mphi \rightarrow \nexists{\rho}~\rho \models \phi$. 
%\end{lemma}
%
%\begin{proof}
%Assume $\rho \models \phi$, then by lemma~\ref{l:3.0}, $\exists{~\rho'}~\rho' \models \mphi$ which is
%a contradiction to the left hand side of the implication, and thus such a $\rho$ does not exist. 
%\end{proof}
%
%\begin{theorem} \label{th:induction}
% Let $\phi = \psi;x_{n+1}y_{n+1}$ and $\mphi = DFA(\phi)$ then $\exists{\rho}~\rho \models \phi \Leftrightarrow \exists{\rho'}~\rho' \models \mphi$
%\end{theorem}
%
%\begin{proof}
% The proof follows directly from lemmas~\ref{l:3.0} to~\ref{l:3.3}
%\end{proof}

